The Field-based Model: A New Perspective on RF-based Material Sensing

This paper introduces the design and implementation of WiField, a WiFi sensing system deployed on COTS devices that can simultaneously identify multiple wavelength-level targets placed flexibly. Unlike traditional RF sensing schemes that focus on specific targets and RF links, WiField focuses on all media in the sensing area for the entire electric field. In this perspective, WiField provides a unified framework to finely characterize the diffraction, scattering, and other effects of targets at different positions, materials, and numbers on signals. The combination of targets in different positions, numbers, and sizes is just a special case. WiField proposed a scheme that utilizes phaseless data to complete the inverse mapping from electric field to material distribution, thereby achieving the simultaneous identification of multiple wavelength-level targets at any position and having the potential for deployment on a wide range of low-cost COTS devices. Our evaluation results show that it has an average identification accuracy of over 97% for 1-3 targets (5 cm * 10 cm in size) with different materials randomly placed within a 1.05 m * 1.05 m area.

==> figures/scatter.tex <==
\def\globalscale{1.3}
\def\linewidthEz{0.7pt}
\begin{tikzpicture}[y=0.55cm, x=0.8cm, yscale=\globalscale,xscale=\globalscale, inner sep=0pt, outer sep=0pt]

    \tikzstyle{vector} = [->,>=stealth,line width=\linewidthEz]
    
    % Draw the incoming vector E_i
    \draw[vector] (-2.5,2) --node[below,yshift=-5pt] {$\bm{E}_i$} (-1.1,0.5) ;
    
    % Draw the scattered vector E_s
    \draw[vector] (0.75,1) --node[above,yshift=5pt] {$\bm{E}_s$} (2,1.5) ;
    
    % Draw the irregular shape representing the scattering object with label epsilon
    \draw[fill=gray!60!white] plot[smooth cycle, tension=0.7] coordinates {
        (-1,0.5) (0,3) (1,2.5) (0.7,1) (1.2,0) (0.3,-1)
    };
    \node at (0,0) {$\epsilon$};
\end{tikzpicture}

==> sec/intro.tex <==
\section{Introduction}
The interference caused by different static environments severely hinders the deployment and application of wireless sensing systems~\cite{fanFlexibleWirelessCharging2020,liang2021fg,niu2018boosting,zhang2017toward}.
These interferences are mainly influenced by two factors: the shape and material.
At present, camera-based target shape sensing schemes have made significant progress.
However, due to obstructions such as packaging and containers, visual-based schemes struggle to identify target materials in many scenarios~\cite{chang2018rf,zhangWicyclopsRoomscaleWiFi2024}.
Identifying the material of static targets is one of the key issues in wireless sensing.

Due to the ubiquitous characteristic, many artistic systems have explored the possibility of material identification using radio frequency (RF) signals.
For instance, Tagscan~\cite{wang2017tagscan}, LiquID~\cite{dhekne2018liquid}, LiqRay~\cite{shang2022liqray}, WiMi~\cite{fengWiMiTargetMaterial2019}, etc., have achieved high-resolution liquid identification based on sub-6G signals.
However, \textbf{they require the target to be placed in a specific position for identification}, which hinders their application in real-world scenarios.
FG-Liquid~\cite{liang2021fg} and LiquImager~\cite{shangLiquImagerFinegrainedLiquid2024} have realized position-invariant material identification, but \textbf{they can only identify a single target}, while static targets in the environment often have multiple ones.
Wi-Painter~\cite{yanWiPainterFinegrainedMaterial2023} has achieved multi-target identification.
However, \textbf{it requires the target size to be much larger than the wavelength to work well}.
Unfortunately, a large number of targets in the environment have sizes similar to the wavelength of the most widely existing video signal, sub-6G.

In summary, the aforementioned solutions are absent in the following three design properties:
\begin{itemize}
    \item \textbf{Sensing targets anywhere.} Since the position of the target to be identified is changeable, the system can not only identify the target at a specific position.
    \item \textbf{Multi-target sensing.}
    In most environmental species, there is more than one static target, which requires the system to identify at least two targets simultaneously.
    \item \textbf{Near-wavelength target sensing}. Due to the fact that many targets are of similar size to the wavelength of RF signals, the system needs to focus on the sensing of the target with sizes close to wavelength.
\end{itemize}

In this paper, we propose \systemname, a material identification system based on WiFi devices.
The basic idea comes from a observation: different materials have different effects on WiFi signals.
Unlike previous works, which mainly analyze material information from a specific RF link (usually a ray), we try to explore this problem from \textbf{the perspective of the field}.
Specifically, the received signal depends on the distribution of materials in the entire sensing domain.
We want to \textbf{construct a scheme to achieve the mapping from the received signal to the material distribution}.
In this perspective, there is no substantial difference between a single target or multiple targets, or targets in different locations\footnote{There will be differences in the difficulty of solving.}.
As long as we make this scheme suitable for the perception of near-wavelength target objects, we have achieved our goal.
However, it is still difficult to implement field-based sensing on COTS WiFi devices.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/intro2.pdf}
    \caption{Utilizing WiFi signals to identify multiple centimeter-level targets placed randomly.}
    \vspace{-1em}
    \label{fig:challenges}
\end{figure}

(1) \textbf{How to accurately describe the target's impact on WiFi signals?}
The material, position, and shape of the target will all affect the electromagnetic signal, and this information is various. 
In addition, the size of the target to be sensed is often close to the wavelength of the WiFi signal (for example, the wavelength of a WiFi signal with a frequency of \SI{2.4}{GHz} is \SI{12.5}{cm}), which brings obvious diffraction phenomenon. 
All of those effects make common sensing models (such as ray tracing models) inaccurate enough.

(2) \textbf{How to recover the distribution of material from underdetermined signals?}
There are often hundreds or thousands of data to be estimated (for example, if we discretize the sensing domain into a $40 \times 40$ grids, we need to estimate 1600 parameters), and even if we use a MIMO WiFi system, there are only dozens even several independent WiFi links. 

(3) \textbf{How to accurately identify with severe noise?}
We expect to recover the material and shape of the target from the received signal with high resolution.
However, due to the presence of CFO, etc., WiFi data contains severe phase noise, which further reduces the amount of information contained in the received signal.



\textbf{Our solutions are as follows.}
Firstly, we construct a field sensing model based on Maxwell's equations, which can more accurately describe the effects of multi-target diffraction and other factors on RF signals.
In order to use WiFi data with severe phase noise to estimate the distribution of material in the sensing domain, we do not directly solve the equation, but design an optimization method based on relatively stable amplitude data to find the solution that is ``most similar" to the real situation, and introduce the position information of the target as a regularization term to constrain the solution space.
Finally, we design \netname, using the non-linear characteristics of deep learning networks to improve the resolution of the results.

\textbf{Contributions:} The main contributions in \systemname\ summarize as follows:

(1) We design \systemname, which can perform material identification using commercial WiFi devices. To the best of our knowledge, this is the first WiFi sensing system to achieve simultaneously identify multiple near-wavelength targets no matter where they are placed, which will provide more possibilities for ubiquitous sensing.

(2) We construct a field sensing model that finely describes the diffraction and multiple scattering of signals, enabling the sensing of near-wavelength-sized targets. Moreover, we design a material recognition scheme based on phaseless data. Compared to existing WiFi sensing systems that typically rely on multi-antenna characteristics to process phase data, our scheme has lower device dependence, facilitating deployment on a wider range of WiFi devices.

(3) We test \systemname\ in a area of \SI{105}{cm} $\times$ \SI{105}{cm}. For multiple (1-3) targets (5-\SI{10}{cm} in size) randomly placed within, the average accuracy of material identification exceeds 97\%.


The rest of the paper is organized as follows.
In Section~\ref{sec:pre}, we introduce the background of the antenna and Maxwell's equations.
In Section~\ref{sec:model}, based on Maxwell's equations, we build a basic RF sensing model.
We present the overview of our system in Section~\ref{sec:overview}.
We detail how to use the received signal for pre-identifying, the method of image enhancement in Section~\ref{sec:system_design}.
Implementation and evaluation are presented in Section~\ref{sec:imp} and Section~\ref{sec:eva}.
Finally, we discuss the related work in Section~\ref{sec:relatedwork}.
